Fast Localization and Tracking in City-Scale UWB Networks

Localization of networked nodes is an essential problem in emerging applications, including first-responder navigation, automated manufacturing lines, vehicular and drone navigation, asset navigation and tracking, Internet of Things and 5G communication networks. In this paper, we present Locate3D, a novel system for peer-to-peer node localization and orientation estimation in large networks. Unlike traditional range-only methods, Locate3D introduces angle-of-arrival (AoA) data as an added network topology constraint. The system solves three key challenges: it uses angles to reduce the number of measurements required by 4x and jointly use range and angle data for location estimation. We develop a spanning-tree approach for fast location updates, and to ensure the output graphs are rigid and uniquely realizable, even in occluded or weakly connected areas. Locate3D cuts down latency by up to 75% without compromising accuracy, surpassing standard range-only solutions. It has a 10.2 meters median localization error for large-scale networks (30,000 nodes, 15 anchors spread across 14km square) and 0.5 meters for small-scale networks (10 nodes).

==> design.tex <==
\section{System Design}

Localization exists, one of the challenges is they are vey data hungry. With 2-3 nodes they do not perform and their accuracy

% Justify why we are doing and then what/how.

% Primer to talk about 6DoF and orientation

People care about why?

I should identify - Big two/three modules

What is spatial-angle?



1. Optimization algorithm
    New name - 

    Least square approach of MDS cannot incorporate angles
    Optimization algorithm becomes non-convex

    The algo name - Past people have worked on it. MDS fundamental works this way. Howvene when we add angle it does not work.
    Challenge  - 
    maybe subheadings.
    Now we have tthis problem. How we are solving it.


    Figure showing the shortcoming of MDS. Or - Limitation of XYZ (generic) based optimization.
    
    Orientation 
    For the first time use angles and ranges to find 6DoF 
    AoA preprocessing
    Location estimation

    
2. Camera based absolute location estimation




3. Dealing with 
AoA can be unreliable - Limitation of view. In our system it surfaces as this problem. If we have a generic solution - ok.





% Highlight these - 
% Incorporating angles.
% How do we seamlessly integrate.

% Selecting the particular angle.

% 1. Algorithmic - Orientation challenge. 
% 2. System - Have a limited fov, aoa we could potentially get from CIR we could only get in certain range. Not how to use it and when to use it.


% A. Picking edges for LOS/NLOS

We propose \name, a system that uses RF to perform robust 6DOF localization for multi-user applications. This section presents the high-level system overview of \name followed by details of each module.

\subsection{System Overview}

\begin{figure}
    \centering
    \includegraphics[width=3.4in]{Figures/system_overview1.pdf}
    \caption{System overview}
    \label{fig:system_overview1}
\end{figure}

Figure \ref{fig:system_overview1} shows the overview of \name.
\name is orchestrated by a central controller which is connected to all the mobile nodes through WiFi or alternate wireless communication link.
The controller requests the nodes to perform measurements with each other and send back range, azimuth and elevation angles to the controller. The controller collects multiple measurements of various nodes and computes a topology of nodes where each connecting edge denotes a measurement. Figure \ref{fig:system_overview2} shows an example topology where the lines denote performed measurements. The solid lines denote line-of-sight (LOS) edges and dashed lines denote non-line-of-sight (NLOS) edges. The system classifies an edge as LOS or NLOS based on the channel impulse response (CIR) of the UWB range measurements. The same CIR is also used to get the azimuth and elevation AoA for each node.
Using the collected range and AoA measurements the controller estimates the 3D location and orientation for each node and communicates the results back the nodes. The nodes can then use this location and opportunistically fuse their local VIO measurements to get a fine-grained trajectory in real-time.


% \begin{figure}
%     \centering
%     \includegraphics[width=3.1in]{Figures/topology_example.png}
%     \caption{topology_example}
%     \label{fig:topology_example}
% \end{figure}

\subsection{6 Degrees of Freedoms - Location \& Orientation}

3D location of a node can be represented in either cartesian coordinates $(x,y,z)$ or spherical coordinates $(r, \theta, \phi)$ which correspond to distance, azimuth angle and elevation angles of a 3D point respectively. Figure \ref{fig:spherical_euler_angles} (a) shows the representation of a node localised using spherical coordinates. Here 

\begin{figure}
    \centering
    \includegraphics[width=1.6in]{Figures/spherical_coordinates.png}
    \includegraphics[width=1.6in]{Figures/euler_angles.png}
    \caption{(a) Location of node represented using spatial angles $\theta$ and $\phi$ (azimuth and elevation) and range. (b) Orientation of node represented using euler angles $\alpha$, $\beta$ and $\gamma$ (roll, pitch and yaw) around the X, Y and Z axis respectively.}
    \label{fig:spherical_euler_angles}
\end{figure}

The 3D orientation of the node can be represented using three rotation angles. In this paper, we use euler angles $(\alpha, \beta, \gamma)$ which represent a node's rotation around its X, Y and Z axis respectively. These angles are also called Roll, Pitch and Yaw of the node. It's important to note that when we use euler angles, the order of rotation matters. In this work, we use the \textit{Z-Y-X} sequence, where the node first rotates around the Z axis, then the Y axis, and finally the X axis. Figure \ref{fig:spherical_euler_angles} (b) shows an illustration of euler angles to show the orientation of the node.

\subsection{3D Orientation Estimation}

When wireless signals are received by the UWB array of a node, the AoA is measured in the array’s local frame of reference. The local frame of reference is fixed for the node and rotates with the node’s orientation in a global frame of reference. Our goal is to compute the node’s orientation in a global frame of reference using the measured AoAs in local frame of reference. We treat one of the node in the topology as the origin of the global coordinate system, which has all 0 orientation angles.
\new


%Any 3D rotation of a node can be composed of a combination of three individual rotations around the x, y and z basis axes. For example, we can rotate a node in any direction using a sequence of three rotations: $V = R_{z}(\gamma)R_{y}(\beta)R_{x}(\alpha) U $, where $R$ is a 3 by 3 rotation matrix around a basis axes and $V$ and $U$ are the 3D unit vectors of the initial and rotated coordinates.



We obtain the roll $(\alpha)$ and pitch $(\beta)$ angles using an accelerometer which gives the direction of gravity. 
To compute the yaw $(\gamma)$ angle, we first update the azimuth and elevation measurements in a way as if they were obtained from nodes with zero roll and pitch angles. 
This process involves rotating the local coordinate systems of each node based on their estimated roll and pitch angles.
Any 3D rotation of a node/vector can be composed of a combination of three individual rotations around the x, y and z basis axes. 
For example, we can rotate a vector in any direction using a sequence of three rotations: $V = R_{z}(\gamma)R_{y}(\beta)R_{x}(\alpha) U $, where $R$ is a 3 by 3 rotation matrix around a basis axes and $U$ and $V$ are the 3D unit vectors before and after the rotation.
\new

% \begin{equation*}
%     \label{eq:rotation_matrix}
%     \begin{gathered}
%         R(\alpha, \beta, \gamma) = 
%         \begin{bmatrix}
%         1 & 0 & 0 \\
%         0 & \cos{\gamma} & -\sin{\gamma}\\
%         0 & \sin{\gamma} & -\cos{\gamma}\\
%         \end{bmatrix}
%         \begin{bmatrix}
%         \cos{\beta} & 0 & \sin{\beta}\\
%         0 & 1 & 0\\
%         -\sin{\beta} & 0 & \cos{\beta}\\
%         \end{bmatrix}\\
%         \begin{bmatrix}
%         \cos{\alpha} & -\sin{\alpha} & 0 \\
%         \sin{\alpha} & -\cos{\alpha} & 0 \\
%         0 & 0 & 1 \\
%         \end{bmatrix}
%     \end{gathered}
% \end{equation*}

%To perform this operation and obtain the AoA measurements in the updated coordinate system, we follow the three steps below:
To obtain the updated AoA measurements, we follow these three steps:

%we first align the local frame to the global frame and align the X-Y planes of both frames. We now compute the new azimuth and elevation angles from this rotated planes [Write the equations for this]. Now azimuth contains yaw orientation information. 
% We use the following $R_{x}$ and $R_{y}$ to first rotate the node in X-Y plane.
%Step1 - Spherical to cartesian [Unit vector from measured azimuth and elevation]

Step1 - Compute the unit vector corresponding to the estimated azimuth and elevation measurements using the following equation:
\[ U = 
\begin{bmatrix}
\hat{x}\\ \hat{y}\\ \hat{z}
\end{bmatrix}
=
\begin{bmatrix}
cos(\phi)*cos(\theta)\\
cos(\phi)*sin(\theta)\\
sin(\phi)
\end{bmatrix}
\]


%Step2 - Rotate the cartesian coordiantes by -beta and -gamma vector
Step2 - Use a rotation matrix to rotate the unit vector by the same roll and pitch angles that we computed earlier using the gravity vector.
\[V = R_{y}(\beta)R_{x}(\alpha) U \]
% \[V = R(\alpha, \beta, 0) U \]

\[V = \begin{bmatrix}
\cos{\beta} & 0 & \sin{\beta}\\
0 & 1 & 0\\
-\sin{\beta} & 0 & \cos{\beta}\\
\end{bmatrix}
\begin{bmatrix}
\cos{\alpha} & -\sin{\alpha} & 0 \\
\sin{\alpha} & -\cos{\alpha} & 0 \\
0 & 0 & 1 \\
\end{bmatrix} U \]

Step3 - The azimuth and elevation angles of the rotated vector V provides the desired AoA measurements, where each node's coordinate system is perfectly aligned with zero roll and pitch angles. 
The following equation can be used to compute the new azimuth and elevation angles of the rotated vector:
%\[\theta = tan^{-1}(y/z), \phi = tan^{-1}(z/\sqrt{x^2 + y^2 + z^2})\]
\[ 
\begin{bmatrix}
\hat{\theta} \\ \hat{\phi}
\end{bmatrix}
=
\begin{bmatrix}
tan^{-1}(y/z)\\
tan^{-1}(z/\sqrt{x^2 + y^2 + z^2})
\end{bmatrix}
\]

% \begin{equation*}
%     \label{eq:rotation_matrix}
%     \begin{gathered}
%         R_{x}(\alpha) = 
%         \begin{bmatrix}
%         \cos{\alpha} & -\sin{\alpha} & 0 \\
%         \sin{\alpha} & -\cos{\alpha} & 0 \\
%         0 & 0 & 1 \\
%         \end{bmatrix},\\
%         R_{y}(\beta) = 
%         \begin{bmatrix}
%         \cos{\beta} & 0 & \sin{\beta}\\
%         0 & 1 & 0\\
%         -\sin{\beta} & 0 & \cos{\beta}\\
%         \end{bmatrix},\\
%         R_{z}(\gamma) = 
%         \begin{bmatrix}
%         1 & 0 & 0 \\
%         0 & \cos{\gamma} & -\sin{\gamma}\\
%         0 & \sin{\gamma} & -\cos{\gamma}\\
%         \end{bmatrix}
%     \end{gathered}
% \end{equation*}


% \begin{equation*}
%     \label{eq:rotation_matrix}
%     \begin{gathered}
%         R(\alpha, \beta, \gamma) = \\
%         \begin{bmatrix}
%         \cos{\alpha} & -\sin{\alpha} & 0 \\
%         \sin{\alpha} & -\cos{\alpha} & 0 \\
%         0 & 0 & 1 \\
%         \end{bmatrix}
%         \begin{bmatrix}
%         \cos{\beta} & 0 & \sin{\beta}\\
%         0 & 1 & 0\\
%         -\sin{\beta} & 0 & \cos{\beta}\\
%         \end{bmatrix}
%         \begin{bmatrix}
%         1 & 0 & 0 \\
%         0 & \cos{\gamma} & -\sin{\gamma}\\
%         0 & \sin{\gamma} & -\cos{\gamma}\\
%         \end{bmatrix}
%     \end{gathered}
% \end{equation*}


% AoA is always measured in local frame of reference. It is a function of the spatial-angle and orientation-angle.

% Spatial-angle is the angle between the edge connecting two nodes and the reference axis in global frame of reference.

% Orientation-angle is the rotation offset around the global axis.

% We can write the measured AoA as

% \begin{equation*}
%     \label{eq:orientation_loss}
%     \begin{gathered}
%         \theta_{global} = \theta_{local} + \alpha
%     \end{gathered}
% \end{equation*}




% Exaplin what is oreintation

% Explain the problem we are trying to solve - what exactly are we trying to estimate. In this example our goal is to meaure the relative change of angle between two nodes which is the azimuth orientation. then this thing direclt applies to 3D.

% Show the intuition on how to do it. Keep rotating until the vectors of orientation align with AoA

% Show some result



% The 3D orientation of a node can be represented using a vector of Euler angles (Roll, Pitch and Yaw). Roll, pitch and yaw are the angles that the node rotates about its X, Y and Z axis respectively. For Euler angles, the order of rotation also matters and in this work, we follow the Z-Y-X sequence, where the node first rotates around Z, then Y and finally X axis. Figure \ref{fig:orientation_example}(b) shows the illustration of rotations using euler angles.
% To represent the 3D orientation of a node, we use a vector of Euler angles (Roll, Pitch, and Yaw). These angles represent the node's rotation around its X, Y, and Z axis respectively. It's important to note that the order of rotation matters when using Euler angles. In this work, we use the Z-Y-X sequence, where the node first rotates around the Z axis, then the Y axis, and finally the X axis. Figure \ref{fig:spherical_euler_angles}(b) shows an illustration of euler angles.

% The measured AoA for a node depends on it's own orientation.
% The measured AoA is not eqaual to the true global angles between the nodes.
% Figure \ref{} shows two cases. First, where the nodes have same orientations with respect to each other. In this case, the global angle is equal to the measured angle. However, in the second case, where the nodes are rotated by some orientation angle, alpha1 and alpha2, then the global AoA is a function of both AoA and orientation. We aim to jointly solve for both the orientation and global angles using a constraint optimization function.

% The AoA is always measured in a local frame of reference. It is not necessarily equal to the global angle between the nodes. It's value depends on the node's orientation in the global frame of reference.

%Now we have to estimate the yaw orientation angle.




As shown in Figure \ref{fig:orientation_example}, when two nodes are oriented with the global frame of reference which means that the orientation angle is zero, then the measured AoA in the local frame of reference ($\hat{\theta_{i}}, \hat{\theta_{j}}$) is equal to the global angle of the edge connecting the two nodes ($\theta_{i}, \theta_{j}$). However, when these nodes are rotated by arbitrary orientation-angles ($\gamma_{i}$ and $\gamma_{j}$), their measured AoAs changes. It becomes a function of both the measured AoA and their orientation. $\hat{\theta_{i}} = \theta_{i} + \gamma_{i}$

\begin{figure}
    \centering
    \includegraphics[width=3.1in]{Figures/orientation_example.png}
    \caption{Orientation changes the measured AoA. Here is an example in 2D. (a) Both nodes have zero orientation, they are aligned with the global axis. In this case the measured AoA is equal to the true angles between the nodes. (b) In this case the nodes are rotated by alpha1 and alpha2 respectively, hence the measured AoA is not same as true global AoA. We must notice in both cases, the difference in global angles must be 180 degrees. We use this property to design our loss function where we find the optimal orientations of all nodes through minimizing the loss function.}
    \label{fig:orientation_example}
\end{figure}

Formulation of the optimization problem:
Notice that in the first case, when orientation is zero for both the nodes, the measured AoA is equal to the global nodes. And it follows a property to complementary angles. Where the angles subtended from the parallel lines are equal. That is $\theta_{ij} = \pi + \theta_{ji}$. Or $\theta_{ij} - \theta_{ji} = \pi$.
We estimate the orientation angles, $\gamma$, by minimizing the following loss function:

\begin{equation*}
    \label{eq:orientation_loss}
    \begin{gathered}
        \underset{\gamma} {\text{min}} \sum_{i} \sum_{j}
        (\pi - (\theta_{ij} + \gamma_{i}) - (\theta_{ji} + \gamma_{j}))
    \end{gathered}
\end{equation*}

We assume $\gamma_{1} = 0$ and all other orientation are in the reference frame of first node.
After obtaining the orientation-angles of all the nodes, we compute the spatial-angles.

% After estimating orientation of all the nodes, we can simply calculate the global angles by subtracting orientation from measured AoAs.








\subsection{3D Location Estimation}

% A paragraph to tell the overall idea of how we formulate our location estimation problem like an optimization problem.
% Talk about existing classical-MDS method and its alternates based on least square and weighted ones.

MDS (Multidimensional scaling) is a popular technique that is used by existing works to estimate the coordinates of a network of connected nodes. The idea behind MDS is to formulate the problem as least squares optimization problem and minimize the difference between the measured euclidean distances of network and the distances corresponding with the estimated coordinates.
There are several ways to implement MDS, such as classical MDS, metric MDS, non-metric MDS, distributed weighted MDS \cite{}. All these assume a fully connected topology. There are variation which account for missing edges as well \cite{}. Our approach builds on top of these and starts by first formulating our problem as an optimization problem.
\new

\begin{figure}
    \label{eq:}
    \centering
    \includegraphics[width=3.3in]{Figures/loss_functions.png}
    \caption{Visualizing the loss function for a simple two node topology. (a) arctan() (b) arctan2() (c) cosine}
    \label{fig:loss_functions}
\end{figure}

\subsubsection{Problem formulation:}
We consider a topology of N nodes (mobile devices or headsets), with unknown locations $X = [(x_{1}, y_{1}, z_{1}), \cdots (x_{N}, y_{N}, z_{N})]$. Suppose the nodes measure the range between each other, $\hat{r_{ij}}$ where $(i,j)$ is the pair nodes $i$ and $j$ in the topology. We aim to solve for $X$ while minimizing the cost function:
\new

\begin{equation*}
    \label{eq:}
    \begin{aligned}
        \underset{X} {\text{min}} \sum_{i} \sum_{j} w_{ij} (\hat{r_{ij}} - r_{ij}(X))^2
    % \underset{X} {\text{min}} \sum_{i} \sum_{j} w_{ij} (\hat{d_{ij}} - || x_{i} - x_{j} ||)^2
    \end{aligned}
\end{equation*}

where, $w_{ij}$ is the weight assigned to edge between nodes $i$ and $j$ and $r_{ij}(X)$ is the euclidean distance between them given by, $r_{ij}(X) = \sqrt{(x_{i} - x_{j})^2 + (y_{i} - y_{j})^2 + (z_{i} - z_{j})^2}$. We use $w_{ij} = 0$ for missing edges.

% \begin{equation*}
%     \label{eq:}
%     \begin{aligned}
%         d_{ij}(X) = \sqrt{(x_{i} - x_{j})^2 + (y_{i} - y_{j})^2 + (z_{i} - z_{j})^2}
%     \end{aligned}
% \end{equation*}


% \begin{figure*}[htb]
%     \centering
%     \includegraphics[width=6.5in]{Figures/error_percent_of_edges_cdf.pdf}
%     \caption{Localization error for varying \% of edge measured in a topology.}
%     \label{fig:error_percent_of_edges_cdf}
% \end{figure*}


\begin{figure*}[hbt]
\centering
\subfloat[\small{100\% edges}]{\includegraphics[width=1.64in]{Figures/Evaluations/error_percent_of_edges_cdf_7.pdf}\label{subfig:100edges}}
\hskip1ex
\subfloat[\small{80\% edges}]{\includegraphics[width=1.64in]{Figures/Evaluations/error_percent_of_edges_cdf_5.pdf}\label{subfig:80edges}}
\hskip1ex
\subfloat[\small{70\% edges}]{\includegraphics[width=1.64in]{Figures/Evaluations/error_percent_of_edges_cdf_4.pdf}\label{subfig:70edges}}
\hskip1ex
\subfloat[\small{50\% edges}]{\includegraphics[width=1.64in]{Figures/Evaluations/error_percent_of_edges_cdf_3.pdf}\label{subfig:50edges}}
\hskip1ex
\caption{Localization error for varying \% of edge measured in a topology.}
\label{fig:error_percent_of_edges_cdf}
\end{figure*}




\begin{figure}[htb]
    \centering
    \includegraphics[width=3.0in]{Figures/error_vs_degree_of_node.pdf}
    \caption{Median localization error for varying degree of nodes.}
    \label{fig:error_vs_degree_of_node}
\end{figure}

% \begin{figure}
%     \centering
%     \includegraphics[width=1.05in]{Figures/topology_example_ground_truth.pdf}
%     \includegraphics[width=1.05in]{Figures/topology_example_ranges.pdf}
%     \includegraphics[width=1.05in]{Figures/topology_example_ranges_angles.pdf}
%     \caption{Topologies (a) Ground truth locations (b) Estimated Locations using ranges only (c) Estimated Locations using ranges and angles}
%     \label{fig:topology_example_range_and_angles}
% \end{figure}

\begin{figure*}[htb]
    \centering
    \includegraphics[width=6.0in]{Figures/topology_example_2d.pdf}
    \caption{Examples of estimated topologies using different optimizations.}
    \label{fig:topology_example_2d}
\end{figure*}

\begin{figure}[hbt]
\centering
\subfloat[\small{Ground truth}]{\includegraphics[width=1.05in]{Figures/topology_example_ground_truth.pdf}\label{subfig:topology_example_ground_truth}}
\hskip1ex
\subfloat[\small{Ranges only}]{\includegraphics[width=1.05in]{Figures/topology_example_ranges.pdf}\label{subfig:topology_example_ranges}}
\hskip1ex
\subfloat[\small{Ranges+angles}]{\includegraphics[width=1.05in]{Figures/topology_example_ranges_angles.pdf}\label{subfig:topology_example_ranges_angles}}
\hskip1ex
\caption{(a) Ground truth topology (b) Estimated topology using ranges only (c) Estimated topology using ranges and angles}
\label{fig:topology_example_range_and_angles}
\end{figure}




\subsubsection{Incorporating angles:}
% To incorporate angles in the topology, we design a new loss function which makes the 
% Angles add more constraints and require less number of edges to solve for 3 dimensional locations.

% We can't use angles directly, It's a highly non convex problem.

% The basic loss function of minimizing error in true angle and calculated angles:

Similar to the range based optimization, consider the following function, $f(X)$, which formulates the difference between measured angles, $\hat{\theta_{ij}}$, and estimate angles.

\begin{equation*}
    \label{eq:loss_1}
        % \lambda_{1}(X) = \Big[ \hat{\theta_{ij}} - \text{arctan}(\frac{\Delta y_{ij}}{\Delta x_{ij}}) \Big] ^2
        f(X) = \Big[ \hat{\theta_{ij}} - \text{arctan}\Big[\frac{y_{i} - y_{j}}{x_{i} - x_{j}}\Big] \Big] ^2
\end{equation*}

When the loss function is visualised for a two node system in Figure \ref{fig:loss_functions} (a), we see that the function is highly non-convex and has discontinuities in the gradient. This is due to two reasons. First, the arctangent function used to calculate the angle only returns angles in the interval of $[-\pi/2, \pi/2]$ and it does not take care of the points in the left quadrants of the plane which results in the same angle for $(x, y) and (-x, -y)$. To take care of this, we use the $arctan2()$ function \cite{}, which is a four quadrant inverse tangent that takes x and y as arguments and takes care of the signs thereby returning angles in the interval $[-\pi, \pi]$. The loss function with $arctan2()$ is visualised in Figure \ref{fig:loss_functions} (b).
\new


Existing solutions \cite{} which use L1 and L2 losses directly on this loss function show that even with an iterative approach the optimizer is likely to get stuck in local minimas.

% \begin{equation*}
%     \label{eq:loss_2}
%         % \Bigg[ \theta - 2atan(\frac{\Delta y_{ij}}{\sqrt{\Delta y_{ij}^2 + \Delta y_{ij}^2} + \Delta x_{ij}}) \Bigg] ^2
%         f_{2}(X) = ( \hat{\theta_{ij}} - \text{arctan2}(y_{i} - y_{j}, x_{i} - x_{j} ) ) ^2
% \end{equation*}

To make the function convex, we design the loss as negative cosine of the angles. 
We take the cosine of the difference of angles, which makes the loss function continuous, differentiable and limited in the range $[0, 1]$. Figure \ref{fig:loss_functions} (c) shows the gradient visualization for the new loss function.

\begin{equation*}
    \label{eq:orientation_loss}
        % 1 - cos \Bigg[ \theta - 2atan(\frac{\Delta y_{ij}}{\sqrt{\Delta y_{ij}^2 + \Delta y_{ij}^2} + \Delta x_{ij}}) \Bigg]
        f(X) = 1 - cos ( \hat{\theta_{ij}} - arctan2(y_{i} - y_{j}, x_{i} - x_{j} ) )
\end{equation*}

Finally, we use $f(X)$ as our angular loss function and add it with the range loss function to formulate a joint optimization problem.

% \begin{equation*}
%     \label{eq:}
%     \begin{aligned}
%         \underset{X} {\text{min}} \sum_{i} \sum_{j} w'_{ij} (1 - cos(\hat{\theta_{ij}} - \theta_{ij}(X)))
%     \end{aligned}
% \end{equation*}

% \begin{equation*}
%     \label{eq:}
%     \begin{aligned}
%         \theta_{ij}(X) = \text{arctan2}(y_{i} - y_{j}, x_{i} - x_{j})
%     \end{aligned}
% \end{equation*}

% \subsubsection{Ranges and angles combined:}
% Range and angle joint optimization.

\begin{equation*}
    \label{eq:}
    \begin{aligned}
        \underset{X} {\text{min}} \frac{\sum_{i} \sum_{j} w_{ij} (\hat{r_{ij}} - r_{ij}(X))^2}{\sum_{i} \sum_{j} \hat{r_{ij}}} + \\
        \sum_{i} \sum_{j} w'_{ij} (1 - cos(\hat{\theta_{ij}} - \theta_{ij}(X)))
    \end{aligned}
\end{equation*}

where, $\theta_{ij}(X) = arctan2(y_{i} - y_{j}, x_{i} - x_{j})$. Note that we scale the range loss function with $(\sum_{i} \sum_{j} \hat{r_{ij}})$. The range loss can be much higher compared to the angular loss, which are in the range $[0, 1]$, and can dominate the overall gradient/overshadow the angular loss. Hence, we normalize the range loss function before adding the angular loss part.
\new

We ran simulations to test the advantage of using angles along with ranges. Figure \ref{fig:error_percent_of_edges_cdf} shows the CDF of localization error for (i) angles only loss function, (ii) ranges only loss function, (iii) angles and ranges combined. We see that the angles that adding angles is beneficial when the topology is not completely connected or measured. In case of 50\% of edges, the ranges based system has median percentile errors greater that 2 meters while angles+ranges based system has <0.5 meters of median error. We also show the median error with increasing number of edges per node (degree of node) in Figure \ref{fig:error_vs_degree_of_node}. This shows that if there are more than 3 edges per node, the ranges and ranges+angles based systems perform equally well. The angles help in constraining the topology when the degree of node is three or less.
A few example 2D and 3D topologies used in the simulation are visualised in Figure \ref{fig:topology_example_range_and_angles} and Figure \ref{fig:topology_example_2d}.
\new

\subsection{Dealing with AoA uncertainty prediction}
Our above solution assumes that the angles are always available for the measured edges. In practice however, the field-of-view of the antenna arrays is limited.

Give examples of different commodity off the shelf UWB modules
Decawave, murata, etc..

The field of view is usually limited between 90 to 120 degrees.

It is to maintain a fair amount of accuracy in measured AoA.


% One of the practical challenge that we face in using angles is the limited field of view that we get from commodity array based UWB devices.

The AoA estimation algorithm uses phase difference of the signal which is a function of sin() of the AoA which results in higher error when the AoA is close to $+\/-90^\circ{}$. Due to this most of the commodity array based modules restrict the AoA field of view to either $-45^\circ{} to +45^\circ{}$ or $-60^\circ{} to +60^\circ{}$. Beyond these field of view the AoA is either saturated or randomly erroneous. We show this example in Figure \ref{} where the estimated AoA is only reliable in the $90^\circ{}$ field-of-view. We require a way to know when the AoA is valid and can be used in the algorithm. Otherwise using a wrong values does more harm by misguiding the direction of optimization function.

We leverage the natural human motion to correlate the time series data of orientation 

We use these additionally sensor modality for example an IMU which will be readily availability in most devices. 


Method of flagging angles.

Add a figure to show VIO correlation with orientation and tell that we only pick angles if it matches. [means flag it]
% \subsection{Picking edges to measure for next iteration}

\subsection{Leveraging oracle view point}
% \subsection{Absolute localization using virtual anchors}
While our system does not require a static anchor it can still use the availability of a static anchor to convert the relative coordinates of the nodes to global coordinates using a known anchor location and orientation.

Since, we also have angles, and not just ranges, we can get the absolute 3 D locations and orientations using just one single anchor. Whereas ranges only system would require atleast 3 anchors which can be hard to find in highly mobile settings.

Trajectory correlation with all possibilities of angle and ranges.

Natural human motion including standing, walking (slow, regular and fast paced).

Talk about the heading direction cosine similarity and the maginitude of motion thing.

Add a figure showing how we correlate trajectories to match virtual anchors and how long it takes. Take existing results.

\begin{figure}[htb]
    \centering
    \includegraphics[width=3.0in]{Figures/users_registration_depiction1.pdf}
    \caption{Scenario of users visible to a static anchor.}
    \label{fig:users_registration_depiction1}
\end{figure}

\begin{figure}[htb]
    \centering
    \includegraphics[width=3.0in]{Figures/users_registered_time_vs_threshold.pdf}
    \caption{Time taken to register users for different threshold of trajectory matching.}
    \label{fig:users_registered_time_vs_threshold}
\end{figure}

\begin{figure}[htb]
    \centering
    \includegraphics[width=3.0in]{Figures/users_registered_vs_threshold.pdf}
    \caption{Percent of users correctly registered for different thresholds of trajectory matching.}
    \label{fig:users_registered_vs_threshold}
\end{figure}


\begin{figure}[hbt]
\centering
\subfloat[\small{Time take}]{\includegraphics[width=1.6in]{Figures/users_registered_time_vs_threshold.pdf}\label{subfig:users_registered_time_vs_threshold}}
\hskip1ex
\subfloat[\small{Percent of users}]{\includegraphics[width=1.6in]{Figures/users_registered_vs_threshold.pdf}\label{subfig:users_registered_vs_threshold}}
\hskip1ex
\caption{User registered for different thresholds of trajectory matching.}
\label{fig:User_registeration}
\end{figure}


\subsection{Opportunistic integration with VIO}
Each node gets a fine grained 3D tracking using on device VIO. We fuse it to get a more fine grained trajectory.


We opportunistically use VIO when available but \name can rely only on RF to get 3D locations and orientations.

\begin{figure}
    \centering
    %\includegraphics[width=3.1in]{Figures/fov_feasibility.png}
    \includegraphics[width=3.1in]{Figures/fov_feasibility.pdf}
    \caption{caption}
    \label{fig:fov_feasibility}
\end{figure}

==> intro.tex <==
\section{Introduction}

% battery free sensors are being scattered - in vast regions
% Miniaturized devices are emerging and platforms are ready to take on sensing and computing together.
% take localization to the next granularity and next level.
% It can trigger a next application and something that was promised but never fulfilled
% Idea -In a vast region scattered sensors can tell each others locations and at the same time it can enable city scale tracking a
% City evacuation - Maui Hawaii
% Not only a building scale but also general movement of animals in large areas
% Sensing techniques and platforms are read
% A big leap of jump will require advanced techniques for 
% 5G is promising deeper IoT and smart cities  where every single public buttons and sewage and storm water drain is connected to network
% Maintainability of all
% The - Now the first thing is can existing techniques be scale to solve this problem
% Fundamental limitation A B C D
% We are solving it in this way
% We took a both theoretical and practical approach/implementation that actually gives the confidence to the entire system.


In recent developments, miniaturized sensors are being dispersed over extensive areas, marking a significant step forward in environmental and urban monitoring. These miniaturized devices are evolving into platforms that combine sensing and computing capabilities, setting the stage for ....

An important feature of this technological shift is the enhancement of localization technologies, moving towards a finer granularity and higher level of sophistication. Through systems where mobile sensors can interact to ascertain each other's positions, a new frontier in city-scale tracking is becoming feasible.
This capability also opens avenues for monitoring animal movement across extensive geographical spans.
For example, in disasters like the recent wildfires in Maui, Hawaii \cite{}, these advancements could have been of helped in city evacuation strategies.
By employing a network of sensors, real-time data on population and asset movement can be harvested to formulate dynamic evacuation plans during emergencies, thus promising a better level of preparedness.
Furthermore, this technological shift aligns well with the deployment of 5G networks, which predicts a future where the building blocks of the city, including lamp posts and drainage systems, are connected to the network.

Fundamental challenges A B C

In this paper we ask, what does it take to  facilitate large-scale 6DoF (six degrees of freedom) localization and orientation. The current state-of-the-art in distributed localization systems falls short of offering such capabilities in a scalable and real-time manner. Addressing this gap represents a key contribution of our approach, blending theoretical analysis and practical implementation 

We present \name, a system that is grounded on both theoretical and practical foundations, providing a reliable framework for the development of systems capable of real-time, large-scale 6DoF localization and orientation. This paper..

Unfortunately, while numerous distributed localization systems have emerged, they all lack the ability to scale to large networks.

The primary technical challenge in this paper lies in reducing the number of edges required to make a rigid and unique graph and at the same time enable 3D orientation estimation.
\new

Our technique significantly reduces the latency by upto $78\%$.


% AR and VR technologies have transformed from being purely for entertainment to becoming integral parts of our daily lives, from shopping for groceries to virtual medical consultations. However, to fully harness the power of these technologies in collaborative and multi-user applications, we need a real-time and accurate 6 degrees-of-freedom (DOF) localization framework.
% \new

% \begin{figure}
%     \centering
%     \includegraphics[width=3.3in]{Figures/system_overview2.pdf}
%     \caption{System overview.}
%     \label{fig:system_overview2}
% \end{figure}

% % Exisitng vison based works have some practical challenges
% There have been several attempts to the 6DOF (3D location and 3D orientation) multi-user localization problem \cite{}. Some of them use infrastructure based anchors, which requires multiple anchor installations in the space. Infrastructure free works which are based on computer vision like Apple ARKit \cite{} and Google ARCore \cite{} which use cameras for SLAM. While vision-based methods have shown promise, they suffer from practical limitations that hinder their applications. They rely on good lighting conditions and are prone to accumulating error and drifting in poorly-lit environments. Furthermore, these methods require all devices to share an overlap of visual features, which limits their applicability to line-of-sight and room-level scenarios. There is a need for a more robust and versatile 6DOF localization framework that can support a wide range of applications in diverse environments.
% \new

% % RF (UWB) will help
% With the emergence of ultra-wideband (UWB) technology in modern devices, there is potential to develop a robust and practical system that can overcome the limitations of visual-based systems. RF-based systems can offer a promising solution for achieving accurate 6DOF localization in environments where line-of-sight between users is not guaranteed or where lighting conditions may be suboptimal. 
% By leveraging the advantages of UWB, we aim to develop a system that can reliably track the 3D location and 3D orientation of each device, creating a real-time topology of mobile users that can be used for a variety of collaborative applications.
% \new

% % Motivation that we need angles and just ranges are not enough
% Wireless network localization is a problem that has received a lot of attention in research \cite{di2017calibration}, with many works focusing on finding the locations of distributed wireless nodes using a set of measurements of edge lengths, or ranges, of the graph.
% UWB has emerged as a popular choice for measuring these ranges due to its high resolution and low power consumption, and recent works have used UWB sensors to perform 3D network localization. 
% However, there are two major challenges with using range measurements for localization systems.
% Firstly, ranges alone cannot provide the full 6DOF position of nodes (3D location + 3D orientation). Ranges can only solve for 3D location at the best. Recent works \cite{miller2022cappella} have attempted to opportunistically fuse visual inertial odometry [VIO] with UWB range measurements, offering promise but suffering from similar challenges to vision-based solutions.
% Secondly, the increasing number of nodes in a topology makes getting the minimum three measurements per node a latency challenge, as range measurements are done sequentially to share the wireless channel.
% \new

% % Solution - Introduce angles
% To overcome the challenges, we propose the use of \textit{angles} in topology measurements. Angles between nodes can be obtained as angle-of-arrival (AoA) using an antenna array in the UWB sensor. The phase delay of an incoming signal across the antenna array can be used to determine the AoA of the signal. This approach enables us to compute the orientation of each node, as the AoA is a function of both spatial angles and orientation angles. Furthermore, incorporating angles in the topology adds more constraints to the rigidity of the graph, thus improving localization accuracy. Measuring AoA does not require additional time since the same signal exchanged between nodes for range measurement can also be used to compute the AoA of the signals. With an L-shaped antenna array, we can measure two AoAs, azimuth, and elevation, as well as range in a single shot, adding $3 \times$ more constraints per edge compared to a range-only system.
% \new

% % However, incorporating angles is not trivial
% Although incorporating angles in topology measurements offers a promising solution to the challenges of 6DoF localization, it presents several research challenges. (1) \textbf{Resolving orientation:} We need to resolve the orientation angles and spatial angles from AoA measurements and use the spatial angles in the topology estimation algorithm.
% (2) \textbf{Knowing how to use angles:} Adding spatial angles to the topology estimation algorithm is non-trivial because the least square loss on angles is non-convex, and optimization algorithms can get stuck in local minima \cite{}, preventing convergence to the final topology. We need to develop an efficient and robust optimization algorithm to use angles in the algorithm.
% (3) \textbf{Knowing when to use angles:} The accuracy of the AoA measurements is limited by the field of view of the antenna array. The AoA estimation algorithm uses phase difference of the signal which is a function of sin() of the AoA which results in higher error when the AoA is close to $\pm90^\circ{}$. Due to this limitation, most commodity array-based modules restrict the AoA field of view to either $-45^\circ{}$ to $+45^\circ{}$ or $-60^\circ{}$ to $+60^\circ{}$. We need to develop a way to identify when the AoA measurement is valid and can be used in the system, as using incorrect values can misguide the direction of the optimization function. We illustrate this example in Figure \ref{}, where the estimated AoA is reliable only in the $90^\circ{}$ field of view. 
% \new

% % Overview of techniques solving the above challenges
% \textbf{\name:} We propose \name, the first RF based 6DOF localization framework that introduces angles in a network of nodes ...
% Give solution to all the three challenges that we have mentioned in the above paragraph.
% Our goal here is to make RF as good as possible using UWB and see how well can it do for a infra-free 6DOF localization system.


% % Overview of system - the high level pitch
% Our core contribution is to make RF better to let it be as good as possible for a VIO like system. Trying to squeeze RF and still using additional modalities like VIO and infrastructure to help in complement.

% % Paragraph to tell that we can opportunistically fuse with VIO or take help of static camera anchors.

% % Summary of prototype and implementation


% % Summary of evaluations and results


% % Summary of contributions
% In summary, our contributions in this work are the following:
% \begin{itemize}
%     \item Incorporating angles. How do we seamlessly integrate? It's not trivial because a) We need to get orientation of individual nodes first. b) We need a new way to use angles in the optimization. Can't simply add angles loss to range loss.
%     \item System level - The arrays have a limited fov for aoa we could potentially get from CIR we could only get in certain range. Not how to use it and when to use it.
%     \item Picking edges in the topology. Things like LOS/NLOS weightage.
% \end{itemize}




% Contributions on algorithms
% Fusion with VIO and infra cameras
% Network level/collaborative works are there

% Our core contribution is making RF better to let it be as good as possible for a VIO like system. Trying to squeeze RF and still using additional modalities like VIO and infrastructure to help in complement.





% We can bank on the idea of developing a platform for UWB 3D localization

% Incorporating the angles is our core contribution. Mainly maximizing the capability of UWB.

% Then showing the application with fusion of other modalities.

% One way is to identify a couple of application. And show performance with VIO one.

% Anything that relies on immersive context applications.

% Although the resolution is good,. It’s currently more dead reckoning approach, it’s hard to rest in one global frame of reference.

% While it has benefits, we can be more robust with global frame of reference..
% RF ha been there for a while…

% We now have the capability of RF with UWB, much more in the useful regime., 

% The works haven’t gone to 3D.

% The is one of the first works that builds RF based infrastructure free localization system that brings contribution at algorithm and system level.

% We also justify with an application fusing vio to show how much we can benefit in los, dim and complex environments.



% Architecture has various layer.

% First is UWB in todays advices.
% This is the basic layer throughout the infra-less 
% Infra can help that is going to global coordinate system.





% Multi-user collaborative AR/VR applications are becoming popular. Existing multi-user tracking relies heavily on visual odometry. Recent work Cappela \cite{} tries to solve the problem by jointly solving a particle filter in VIO+UWB state space but fails when VIO module is absent or cannot track features in dim lit environments. (Motivate the need of UWB over VIO only systems). 


% Expanding the AR/VR space and FOV with RF+vision fusion.

% While existing controllers use only vision they are restricted to a room level application. For a immersive experience and unrestricted access, we need to cover a world level scale. But there is not enough infrastructure, the controller is not there everywhere. So we use RF to make a peer-to-peer network of devices to localize them. It’s a more decentralized approach at some level.

% Now the challenges are:

% 1. Only a few nodes are visible in the camera, how to find other nodes location? Solution - Use RF.
% 2. The nodes might be shortlived where new nodes are entering and exiting a space. We should still be able to carry on with the XR experience.
% 3. The UWB nodes are slow to measure range. In a dense network, we can’t afford to measure all the edges of the node graph. Solution - Use angles to add more constraints and measure less edges to save time and still achieve same accuracy.
% 4. The graph is not absolute it has unknown rotation, translation and mirror image. Solution - Use the nodes visible in the camera as virtual anchors. Use these virtual anchors to peg the graph.
% 5. The controller get ranges from UWB and accurate aoa from camera. How to match the node label of range with node label with aoa? Solution - Use IMU trajectory to match the relative trajectories using all possible ranges and angles.

==> motiv.tex <==
\section{Motivation}
\label{sec:motiv}

\nsdinakul{\textbf{Large scale localization:} With large number of distance measurements between all pairs of nodes in 3D space, it is straightforward to estimate the relative locations of all nodes in the network.
However, the current latency issue in measuring large number of edges, which takes minutes for >400 node network, needs to be addressed to foster a real-time large-scale system.
Incorporating angles to the edges connecting the nodes imposes added constraints in the topology, thereby drastically reducing the number of edges needed to create a \textit{rigid} and \textit{unique} graph.
The angle-of-arrival approach also gives more information to calculate the relative 3D orientations between nodes.
Note that to uniquely determine the node's location, it requires at least three edges per node in a 2D space and four edges in a 3D space.
In contrast, systems that utilize both range and angle data can achieve the same with just a single edge per node, optimizing the latency.
Figure \ref{fig:graphs_comparison_example} presents a comparison of a 200-node topology localized using the ranges-only method and a combination of ranges and angles method.}
\new

\begin{figure}[tb]
    \centering
    \includegraphics[width=3.2in]{Figures/graphs_comparison_example.pdf}
    \caption{Adding angles to the edges between nodes introduces additional constraints to the topology, significantly decreasing the number of edges necessary to achieve a \textit{rigid} and \textit{unique} graph realization. Furthermore, this provides more information to accurately estimate the relative 3D orientations between nodes.}
    \label{fig:graphs_comparison_example}
\end{figure}

\textbf{Why RF?} Existing vision based solutions use VIO. VIO drifts when the visual features are low. For example in dark environments with low lighting conditions or plain environments like a mono color wall. Figure \ref{fig:feasibility_dark} shows the localization errors and a trajectory of a node in well-lit vs dark environment. We see that when the scene gets dark the visual features are lost and VIO begins to drift rapidly increasing the localization error to more than 2 meters within 5 seconds. Such conditions can also happen if the user keeps the phone in pocket or covers the camera's field of view.
\new

\begin{figure}
    \centering
    \includegraphics[width=1.6in]{Figures/Evaluations/feasibility_dark_error.pdf}
    \includegraphics[width=1.6in]{Figures/Evaluations/feasibility_dark_trajectory.pdf}
    \caption{Localization tests for VIO (Visual Inertial Odometry) and UWB (Ultra-Wideband) in varying lighting conditions. (a) The result shows that the VIO system experiences drift and decreased accuracy in darker environments. (b) The result shows the path trajectories during the experiment.}
    \label{fig:feasibility_dark}
\end{figure}

\textbf{Infrastructure-free localization} While there are many localization works that rely on infrastructure, the literature is sparse on infrastructure free mutli-user localization. The VIO based solutions rely on shared visual features to combine the relative trajectories. Hence they suffer from NLOS cases and poor lighting issues. In our system, we use UWB to measure the ranges between the nodes and create a topology/graph of nodes constrained by the measured ranges. Then we estimate the locations of the nodes by solving for the the constraints and optimizing the error. Naturally, the performance increases for topologies with more constraints i.e., more number of edges.
\new

\textbf{Ranges alone are not enough} - While RF solves the problem of poor lighting conditions and multi-user localization, it has its own limitations. Firstly, angles enables us to estimate the complete 6DOF pose (3D coordinates and 3D orientations) of the node. With a range-only based topology, we cannot solve for the orientation of the nodes and again have to rely completely on IMU or odometry based systems.
\new

Additionally, it takes considerable time (around 100-200 ms) to measure the ranges. It is due to limited available channels in low power modules, the MAC layer schedules the range operations in time. While this works well for small network of nodes, the time exponentially increases with large topologies. Figure \ref{fig:time_vs_num_of_nodes} shows the time taken to measure the range for a topology with increasing number of nodes. We clearly see that the time increases exponentially, making the system infeasible for real time applications. In this work, we use UWB antenna arrays to measure both ranges and angles in a single shot. We use the same Channel Impulse Response (CIR) to measure both range and angle. This increases the number of constraints in a topology without costing more time.
\new

% \textbf{Feasibility:} Why we need angles? Ans- To solve for 6DOF, (3D coordinates and 3D orientations) we need many constraints and connected edges. With limited number of edges present in a topology, a traditional range only based system cannot solve for all the unknowns. 
% Furthermore, even in a fully connected topology, it takes considerable time (around 100-200 ms) to measure the ranges. It is due to limited available channels in low power modules, the MAC layer schedules the range operations in time. While this works well for small network of nodes, the time exponentially increases with large topologies. In this work, we use UWB antenna arrays which can measure both ranges and angles in a single shot using the same Channel Impulse Response (CIR) to get ore constraints in limited measurements. However, there are no available techniques to incorporate both angle and ranges in a practical setting for multi node topology.


% Add figure of NLOS showing that VIO is better in NLOS case where UWB is a bit more noisy
